ALDER: Unlocking blockchain performance by multiplexing consensus protocols

Most of today's online services (e.g., social networks, search engines, market places) are centralized, which is recognized as unsatisfactory by a majority of users for various reasons (e.g., centralized governance, censorship, loss of control over personal data). Blockchain technologies promise a new Web revolution (Web 3.0) through the decentralization of online services. However, one of the key limitations for this revolution to happen at a planetary scale is the poor performance of today's blockchains. We propose in this paper ALDER, a solution for unlocking the performance of off-the-shelf leader-based blockchains by multiplexing their consensus protocol. Our solution leverages the existence of multiple potential leaders to alleviate the bottleneck that exists at different levels of consensus protocols. To illustrate the benefits it brings to Blockchain performance, we apply ALDER to three representative blockchains, namely Algorand (Proof-of-Stake), RapidChain (Sharding-based) and Bitcoin (Proof-of-Work). Our evaluation, involving up to 10,000 nodes deployed on 100 physical machines, shows that using ALDER can provide up to a 300% improvement in both throughput and latency reduction.

==> section/background_motivations.tex <==
\section{Background and Motivation}
Throughput issues of Bitcoin,
Transactions propagation,
Propagation of big blocks..
